Analogous Dynamics of Boolean Network

Different Boolean networks may reveal similar dynamics although their definition differs, then preventing their distinction from the observations. This raises the question about the sufficiency of a particular Boolean network for properly reproducing a modeled phenomenon to make realistic predictions. The question actually depends on the invariant properties of behaviorally similar Boolean networks. In this article, we address this issue by considering that the similarity is formalized by isomorphism on graphs modeling their dynamics. The similarity also depends on the parameter governing the updating policy, called the mode. We define a general characterization of the group of isomorphism preserving the mode. From this characterization, we deduce invariant structural properties of the interaction graph and conditions to maintain an equivalence through mode variation.

==> equivfig.tex <==
\begin{center}
\begin{tikzpicture}[baseline,xscale=2.2,yscale=1.5]
\GraphInit[vstyle = normal]
\tikzset{VertexStyle/.style = {
 draw, shape = rectangle,line width = 0.5,inner sep = 2.5pt,outer sep = 0.5pt,minimum size = 0,color = black,fill=white,font=\tiny,text = black }}
\SetUpEdge[style={bend right, post,->}, labelstyle={font=\footnotesize, sloped}]
%%VERTICES
\definecolor{col0000}{rgb}{0.85, 0.85, 0.85} \tikzset{VertexStyle/.append style={fill=col0000}}
\Vertex[x=2.00003,y=-3.16669]{0000}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=2.00003,y=-2.16669]{0001}
\Vertex[x=3.00003,y=-3.16669]{0010}
\Vertex[x=3.00003,y=-2.16669]{0011}
\definecolor{col0100}{rgb}{0.75,0.75,0.75} \tikzset{VertexStyle/.append style={fill=col0100}}
\Vertex[x=0.333343,y=-3.33334]{0100}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=0.333343,y=-2.33334]{0101}
\definecolor{col0110}{rgb}{0.75,0.75,0.75} \tikzset{VertexStyle/.append style={fill=col0110}}
\Vertex[x=0.333343,y=-1.33334]{0110}
\tikzset{VertexStyle/.append style={fill=white}}
\definecolor{col0111}{rgb}{0.75,0.75,0.75} \tikzset{VertexStyle/.append style={fill=col0111}}
\Vertex[x=0.333343,y=-0.333343]{0111}
\tikzset{VertexStyle/.append style={fill=white}}
\definecolor{col1000}{rgb}{0.75,0.75,0.75} \tikzset{VertexStyle/.append style={fill=col1000}}
\Vertex[x=1.33334,y=-3.33334]{1000}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=1.33334,y=-2.33334]{1001}
\definecolor{col1010}{rgb}{0.75,0.75,0.75} \tikzset{VertexStyle/.append style={fill=col1010}}
\Vertex[x=1.33334,y=-1.33334]{1010}
\tikzset{VertexStyle/.append style={fill=white}}
\definecolor{col1011}{rgb}{0.75,0.75,0.75} \tikzset{VertexStyle/.append style={fill=col1011}}
\Vertex[x=1.33334,y=-0.333343]{1011}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=2.00003,y=-1.33334]{1100}
\Vertex[x=2.00003,y=-0.333343]{1101}
\Vertex[x=3.00003,y=-1.33334]{1110}
\definecolor{col1111}{rgb}{0.85,0.85,0.85} \tikzset{VertexStyle/.append style={fill=col1111}}
\Vertex[x=3.00003,y=-0.333343]{1111}
\tikzset{VertexStyle/.append style={fill=white}}
%% EDGES
\Edge[](0001)(0000)
\Edge[](0010)(0000)
\Edge[](0011)(0000)
\Edge[](0100)(1000)
\Edge[](0101)(0110)
\Edge[](0101)(1001)
\Edge[](0110)(0100)
\Edge[](0110)(1010)
\Edge[](0111)(0110)
\Edge[](0111)(1011)
\Edge[](1000)(0100)
\Edge[](1000)(1011)
\Edge[](1001)(0101)
\Edge[](1001)(1011)
\Edge[](1010)(0110)
\Edge[](1010)(1011)
\Edge[](1011)(0111)
\Edge[](1100)(1111)
\Edge[](1101)(1111)
\Edge[](1110)(1111)
\end{tikzpicture} 


\begin{tikzpicture}[baseline,xscale=2.2,yscale=1.5]
\GraphInit[vstyle = normal]
\tikzset{VertexStyle/.style = {
 draw, shape = rectangle,line width = 0.5,inner sep = 2.5pt,outer sep = 0.5pt,minimum size = 0,color = black,fill=white,font=\tiny,text = black }}
\SetUpEdge[style={post,->}, labelstyle={font=\footnotesize, sloped}]
%%VERTICES
\definecolor{col0000}{rgb}{0.8, 0., 0.} \tikzset{VertexStyle/.append style={fill=col0000}}
\Vertex[x=2.00003,y=-3.16669]{0000}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=2.00003,y=-2.16669]{0001}
\Vertex[x=3.00003,y=-3.16669]{0010}
\Vertex[x=3.00003,y=-2.16669]{0011}
\Vertex[x=0.333343,y=-3.33334]{0100}
\Vertex[x=0.333343,y=-2.33334]{0101}
\Vertex[x=0.333343,y=-1.33334]{0110}
\definecolor{col0111}{rgb}{0.9, 0.756, 0.} \tikzset{VertexStyle/.append style={fill=col0111}}
\Vertex[x=0.333343,y=-0.333343]{0111}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=1.33334,y=-3.33334]{1000}
\Vertex[x=1.33334,y=-2.33334]{1001}
\definecolor{col1010}{rgb}{0.9, 0.756, 0.} \tikzset{VertexStyle/.append style={fill=col1010}}
\Vertex[x=1.33334,y=-1.33334]{1010}
\tikzset{VertexStyle/.append style={fill=white}}
\Vertex[x=1.33334,y=-0.333343]{1011}
\Vertex[x=2.00003,y=-1.33334]{1100}
\Vertex[x=2.00003,y=-0.333343]{1101}
\Vertex[x=3.00003,y=-1.33334]{1110}
\definecolor{col1111}{rgb}{0.704, 0.32, 0.8} \tikzset{VertexStyle/.append style={fill=col1111}}
\Vertex[x=3.00003,y=-0.333343]{1111}
\tikzset{VertexStyle/.append style={fill=white}}
%% EDGES
\Edge[](0001)(0000)
\Edge[](0010)(0000)
\Edge[](0011)(0000)
\Edge[](0100)(1000)
\Edge[](0101)(1010)
\Edge[](0110)(1000)
\Edge[style={post,->,bend right}](0111)(1010)
\Edge[](1000)(0111)
\Edge[](1001)(0111)
\Edge[style={post,->,bend right}](1010)(0111)
\Edge[](1011)(0111)
\Edge[](1100)(1111)
\Edge[](1101)(1111)
\Edge[](1110)(1111)
\end{tikzpicture} 




\end{center}
